NP Animacy Identification for Anaphora Resolution

In anaphora resolution for English, animacy identification can play an integral role in the application of agreement restrictions between pronouns and candidates, and as a result, can improve the accuracy of anaphora resolution systems. In this paper, two methods for animacy identification are proposed and evaluated using intrinsic and extrinsic measures. The first method is a rule-based one which uses information about the unique beginners in WordNet to classify NPs on the basis of their animacy. The second method relies on a machine learning algorithm which exploits a WordNet enriched with animacy information for each sense. The effect of word sense disambiguation on the two methods is also assessed. The intrinsic evaluation reveals that the machine learning method reaches human levels of performance. The extrinsic evaluation demonstrates that animacy identification can be beneficial in anaphora resolution, especially in the cases where animate entities are identified with high precision.

==> colortab.tex <==
%% BEGIN colortab.tex/colortab.sty
%%
\def\fileversion{0.9}
\def\filedate{93/01/11}
%%
%% COPYRIGHT 1993, by Timothy Van Zandt, tvz@Princeton.EDU
%%
%% DESCRIPTION:
%%   colortab.tex/colortab.sty lets you shade or color the cells in a
%%   alignment environments (e.g., \halign and \LaTeX's tabular and
%%   array environments). It is compatible with most TeX macro packages,
%%   including Plain TeX, LaTeX, AmSTeX, and Ams-LaTeX. You must be
%%   use in conjunction with other color commands.
%%
%% INSTALLATION:
%%   Put this file where your TeX looks for inputs, under the name
%%   colortab.tex. Name a copy colortab.sty to use as a LaTeX style option,
%%   or create a file colortab.sty with the lines:
%%     \input colortab.tex
%%     \endinput
%%
%% DOCUMENTATION:
%%   See colortab.doc, which might be appended to this file.
%%
%% COPYING:
%%   Copying of part or all of this file is allowed under the following
%%   conditions only:
%%   (1) You may freely distribute unchanged copies of the file. Please
%%       include the documentation when you do so.
%%   (2) You may modify a renamed copy of the file, but only for personal
%%       use or use within an organization.
%%   (3) You may copy fragments from the file, for personal use or for
%%       distribution, as long as credit is given where credit is due.
%%
%%   You are NOT ALLOWED to take money for the distribution or use of
%%   this file or modified versions or fragments thereof, except for
%%   a nominal charge for copying etc.
%%
%% CODE:
%
% colortab.tex uses TeX primitives, plus the Plain TeX commands:
%   \newcount, \newtoks, \newbox, \newif and \z@.
%
% The LaTeX specific macros also use some LaTeX commands.
%
\csname ColortabLoaded\endcsname
\let\ColortabLoaded\endinput
%
\message{\space\space v\fileversion\space\space\filedate\space\space <tvz>}
\edef\TheAtCode{\the\catcode`\@}\catcode`\@=11
%
% These scratch registers are set globally:
%
\newcount\CT@cnt
\newdimen\CT@dim
\newbox\CT@box
%
% This flag is used to shut off colortab:
%
\newif\ifcolortab
\colortabtrue
%
% To color row cells of unknown height we first have to put the rows in an
% alignment and measure the resulting height, then put down a row of blobs
% (with \hrule, and then move back up the page.
%
% For TeX's \halign primitive, \coloralign saves the preamble in the token
% register \CT@preamble. This is used to calculate the height of the columns
% that are to be colored in.
%
\newtoks\CT@preamble
\def\coloralign{%
  \afterassignment\coloralign@
  \setbox\CT@box=\hbox}
\def\coloralign@#1\cr{%
  \egroup
  \CT@preamble{\halign\bgroup#1\cr}%
  \the\CT@preamble}
%
% \CC reads the next row, which should contain the color commands, and then
% the rows to be colored. The height of the latter rows is calculated, and
% then the row of colors is processed. \CT@columncolor uses \leaders to get
% each color to fill the column horizontally, and it uses the previously
% calculated height to fill the columns vertically.
%    \begin{macrocode}
\def\CT@columncolor{%
  \ifx\next\@nil
    \def\next##1&\@nil{\gdef\CT@next{##1}}%
    \expandafter\next\CT@next\@nil
    \def\CT@temp\@nil{}%
  \else
    \ifx\next\CT@space
      \def\CT@temp{%
        \def\next{\futurelet\next\CT@columncolor}%
        \afterassignment\next\let\CT@temp= }%
    \else
      \def\CT@temp{\CT@@columncolor}%
    \fi
  \fi
  \CT@temp}
\def\CT@@columncolor#1&{%
  \ifx\next&%
    \expandafter\gdef\expandafter\CT@next\expandafter{\CT@next\omit{}&}%
  \else
    \expandafter\gdef\expandafter\CT@next\expandafter{\CT@next
      \omit{{\ignorespaces#1{\leaders\hrule height\CT@dim\hfil}}}&}%
  \fi
  \futurelet\next\CT@columncolor}
{\def\\{\global\let\CT@space= }\\ }
\def\CC@#1#2#3{%
  \ifcolortab
    \noalign{%
      \setbox\CT@box=\vbox{#1#3\crcr\egroup}%
      \CT@dim=\ht\CT@box
      \global\advance\CT@dim by \dp\CT@box
      \def\CT@next{}%
      \futurelet\next\CT@columncolor#2&\@nil}%
    \CT@next\cr
    \noalign{\vskip-\CT@dim}%
  \fi
  #3}
\def\CC#1\cr#2\ECC{\CC@{\the\CT@preamble}{#1}{#2}}
%
% With \LaTeX's alignment macros, the preamble is saved for us in \@preamble.
% Otherwise, \LCC is the same as \CC.
%
\def\LCC#1\\#2\ECC{\CC@{\@preamble}{#1}{#2}}
%
% This unaligned color stuff only works with PSTricks:
%
\def\AC#1{%
  \@ifundefined{color@#1}%
    {\@pstrickserr{Color not defined: `#1'}\@ehpa}%
    {\pstVerb{\pst@usecolor{#1}}}}
\def\EAC{\pstVerb{\pst@currentcolor}}
\def\NAC#1{\noalign{\AC{#1}}}
\def\ENAC{\noalign{\EAC}}
%
\def\SP{\noalign{\global\let\CT@savedpreamble\@preamble}}
\def\RP{\noalign{\global\let\@preamble\CT@savedpreamble}}
%
\newcount\CT@LCnum
\def\LColors#1\\{%
  \noalign{%
    \ifnum\CT@LCinitflag=\c@LT@tables\else\CT@LCinit\fi
    \ifnum\CT@LCflag=\z@
      \global\CT@LCnum 1
      \CT@LColors#1&\@nil
      \global\CT@LCnum\CT@LCmax
    \fi}}
\def\CT@LColors#1&{%
  \global\@namedef{LColor@\the\CT@LCnum}{#1}%
  \@ifnextchar\@nil{\@gobble}{%
    \global\advance\CT@LCnum 1
    \CT@LColors}}
\def\CT@LCinit{%
  \ifcolortab
    \@ifundefined{LT@\romannumeral\c@LT@tables}%
      {\gdef\CT@LCflag{1}}{\gdef\CT@LCflag{\z@}}%
  \else
    \gdef{CT@LCflag{1}}%
  \fi
  \ifnum\CT@LCflag=\z@
    \begingroup
      \def\omit\kern##1&{%
        \advance\CT@LCnum 1
        \CT@dim=##1\relax
        \expandafter\xdef\csname LCdim@\the\CT@LCnum\endcsname{%
          \number\CT@dim sp}}%
      \CT@LCnum\z@
      \@nameuse{LT@\romannumeral\c@LT@tables}&%
      \xdef\CT@LCmax{\the\CT@LCnum}%
    \endgroup
  \fi
  \xdef\CT@LCinitflag{\the\c@LT@tables}}
\def\CT@LCinitflag{\z@}
\def\LC@Cell{%
  \kern-\@tempdima
  \ifnum\CT@LCflag=\z@
    \ifnum\CT@LCnum=\CT@LCmax\relax
      \global\CT@LCnum 1
    \else
      \global\advance\CT@LCnum 1
    \fi
    \CT@dim=\@nameuse{LCdim@\the\CT@LCnum}\relax
    \advance\CT@dim-\@tempdimb
    \expandafter\ifx\csname LColor@\the\CT@LCnum\endcsname\@empty\else
      \begingroup
        \@nameuse{LColor@\the\CT@LCnum}{%
        \vrule width\CT@dim}%
      \endgroup
      \kern-\CT@dim
    \fi
  \fi}
\def\LC{\@tempdima=\z@\@tempdimb=\z@\LC@Cell}
\def\LCi{\LCi@\LC@Cell}
\def\LCi@{%
  \@tempdima=\doublerulesep
  \ifnum\CT@LCflag=\z@
    \ifnum\CT@LCnum=\CT@LCmax\relax
      \@tempdimb=\arrayrulewidth
    \else
      \@tempdimb=\z@
    \fi
  \fi}
\def\LCii{%
  \@tempdima=\z@
  \@tempdimb=\doublerulesep
  \advance\@tempdimb=\arrayrulewidth
  \LC@Cell}
\def\LCiii{%
  \LCi@
  \advance\@tempdimb\doublerulesep
  \advance\@tempdimb\arrayrulewidth
  \LC@Cell}
\def\LCz#1#2{%
  \@tempdima=#1
  \@tempdimb=#2
  \LC@Cell}
%
\catcode`\@=\TheAtCode\relax
\endinput
%% END colortab.tex/colortab.sty

